Uncertainty quantification using martingales for misspecified Gaussian processes

We address uncertainty quantification for Gaussian processes (GPs) under misspecified priors, with an eye towards Bayesian Optimization (BO). GPs are widely used in BO because they easily enable exploration based on posterior uncertainty bands. However, this convenience comes at the cost of robustness: a typical function encountered in practice is unlikely to have been drawn from the data scientist's prior, in which case uncertainty estimates can be misleading, and the resulting exploration can be suboptimal. We present a frequentist approach to GP/BO uncertainty quantification. We utilize the GP framework as a working model, but do not assume correctness of the prior. We instead construct a confidence sequence (CS) for the unknown function using martingale techniques. There is a necessary cost to achieving robustness: if the prior was correct, posterior GP bands are narrower than our CS. Nevertheless, when the prior is wrong, our CS is statistically valid and empirically outperforms standard GP methods, in terms of both coverage and utility for BO. Additionally, we demonstrate that powered likelihoods provide robustness against model misspecification.

==> broaderimpact.tex <==
\section*{Broader Impact Statement}
% THIS SECTION CAN GO AFTER PAGE 8

Our work provides a way to perform uncertainty quantification for Gaussian processes using martingales,
with the goal of constructing uncertainty bands that are robust to prior misspecification, 
in order to improve practical performance of Bayesian optimization algorithms.
This work is a level of abstraction away from real applications,
but it can indirectly impact society. Below, we provide a few examples, assuming that our ideas get implemented by practitioners running BO in the real world.

Robust uncertainty quantification can allow for safe exploration
in costly or risky applications of BO, where there are large penalties for mistakes. Further, our tools may allow for 
better-calibrated predictions which are not overly confident in underexplored regions, which may be of
particular importace in high-impact societal applications where the cost of an
erroneous prediction is high. The promising empirical success may help encourage the development of other methods
that are less dependent on potentially biased prior beliefs. Finally, as found in the BO simulations in the supplement, we may actually find better solutions (it does a better job at optimizatiom, the goal of BO), which depending on the underlying application could translate into lower energy consumption, cost-savings, or more equitable distribution of resources.
